Negative Results for Software Effort Estimation

Context:More than half the literature on software effort estimation (SEE) focuses on comparisons of new estimation methods. Surprisingly, there are no studies comparing state of the art latest methods with decades-old approaches. Objective:To check if new SEE methods generated better estimates than older methods. Method: Firstly, collect effort estimation methods ranging from "classical" COCOMO (parametric estimation over a pre-determined set of attributes) to "modern" (reasoning via analogy using spectral-based clustering plus instance and feature selection, and a recent "baseline method" proposed in ACM Transactions on Software Engineering).Secondly, catalog the list of objections that lead to the development of post-COCOMO estimation methods.Thirdly, characterize each of those objections as a comparison between newer and older estimation methods.Fourthly, using four COCOMO-style data sets (from 1991, 2000, 2005, 2010) and run those comparisons experiments.Fifthly, compare the performance of the different estimators using a Scott-Knott procedure using (i) the A12 effect size to rule out "small" differences and (ii) a 99% confident bootstrap procedure to check for statistically different groupings of treatments). Results: The major negative results of this paper are that for the COCOMO data sets, nothing we studied did any better than Boehm's original procedure. Conclusions: When COCOMO-style attributes are available, we strongly recommend (i) using that data and (ii) use COCOMO to generate predictions. We say this since the experiments of this paper show that, at least for effort estimation,how data is collected is more important than what learner is applied to that data.

==> Makefile <==
Src=cocreport-ESE-revised-v1
Name=16emse2
Bib=refs.bib 

all : dirs tex bib  tex tex embedfonts done


publish : dirs all
	cp $(HOME)/tmp/$(Src).pdf pdf/$(Name).pdf
	chmod a+r pdf/$(Name).pdf
	scp -p pdf/$(Name).pdf stuff@ttoy.net:menzies.us/pdf

commit:; - git status; git commit -a; git push origin master
typo:  ; - git status; git commit -am "typo"; git push origin master
update:; - git pull origin master
status:; - git status
gitting:
	git config --global credential.helper cache
	git config credential.helper 'cache --timeout=3600'


view :
	evince $(HOME)/tmp/$(Src).pdf &

one : dirs tex done 

ready :
	mkdir -p $(HOME)/tmp

skim:
	/Applications/Skim.app/Contents/MacOS/Skim $(HOME)/tmp/$(Src).pdf &

done :
	@printf "\n\n\n==============================================\n"
	@printf       "see output in $(HOME)/tmp/$(Src).pdf\n"
	@printf       "==============================================\n\n\n"
	@printf "\n\nWarnings (may be none):\n\n"
	grep arning $(HOME)/tmp/${Src}.log

dirs : 
	- [ ! -d $(HOME)/tmp ] && mkdir $(HOME)/tmp
	- [ ! -d pdf ] && mkdir pdf

tex : ready
	- pdflatex  -output-directory=$(HOME)/tmp $(Src)

embedfonts:
	@ gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite \
          -sOutputFile=$(HOME)/tmp/$(Src)-embedded.pdf $(HOME)/tmp/$(Src).pdf
	@ mv              $(HOME)/tmp/$(Src)-embedded.pdf $(HOME)/tmp/$(Src).pdf

bib : 
	- cp $(Bib) $(HOME)/tmp; cd $(HOME)/tmp; bibtex $(Src)


==> noise.tex <==
% noise

\begin{figure}[!t]
{\scriptsize
{\bf NASA10 (new NASA data up to 2010):}
c
% 0 1 2 3 4 5 6 7 8 9=

{\scriptsize \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{darkgray}
\rowcolor[gray]{.9}  rank & treatment & median & IQR & \\%min= 24, max= 141\\
  1 &      COCOMO-II &    42  &  35 & \quart{0}{29}{15}{64} \\
  1 & COCONUT:c*0.5r=8n/4 &    46  &  36 & \quart{5}{31}{18}{64} \\
  1 &   COCOMO-IIn/2 &    50  &  47 & \quart{0}{40}{22}{64} \\
\hline  
  2 & COCONUT:c*0.5,r=8 &    54  &  34 & \quart{11}{30}{25}{64} \\
  2 & COCONUT:c*0.5,r=8n/2 &    55  &  45 & \quart{0}{39}{26}{64} \\
%  2 &     knear(1) &    57  &  49 & \quart{0}{41}{28}{64} \\
  2 &   COCOMO-IIn/4 &    58  &  45 & \quart{6}{39}{29}{64} \\
%\hline  3 &       cart/4 &    62  &  74 & \quart{10}{63}{32}{64} \\
 % 3 &         cart &    64  &  35 & \quart{19}{30}{34}{64} \\
 % 3 &       cart/2 &    64  &  105 & \quart{10}{89}{34}{64} \\
\end{tabular}}

 %:learn 29.972693 :analyze 3.610701 :boots 5 effects 9 :conf 0.9509900499
% noise


~\\

{\bf COC05 (new COCOMO data up to 2005):}


% 0 1 2 3 4 5 6 7 8 9=

{\scriptsize \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{darkgray}
\rowcolor[gray]{.9}  rank & treatment & median & IQR & \\%min= 16, max= 421\\
 % 1 &         cart &    42  &  57 & \quart{0}{14}{6}{20} \\
%\hline  
1 &      COCOMO-II &    46  &  146 & \quart{0}{37}{7}{20} \\
%  1 &     knear(1) &    55  &  70 & \quart{0}{18}{9}{20} \\
  1 & COCONUT:c*0.5,r=8n/2 &    60  &  53 & \quart{5}{14}{10}{20} \\
  1 &   COCOMO-IIn/2 &    63  &  203 & \quart{2}{50}{11}{20} \\
  1 & COCONUT:c*0.5r=8n/4 &    65  &  42 & \quart{8}{10}{12}{20} \\
 % 1 &       cart/2 &    68  &  55 & \quart{5}{14}{12}{20} \\
  1 & COCONUT:c*0.5,r=8 &    77  &  51 & \quart{6}{12}{15}{20} \\
\hline % 3 &       cart/4 &    82  &  376 & \quart{7}{92}{16}{20} \\
  2 &   COCOMO-IIn/4 &    110  &  280 & \quart{5}{69}{23}{20} \\
\end{tabular}}

 %:learn 366.038237 :analyze 14.041803 :boots 4 effects 4 :conf 0.96059601
% noise

~\\


{\bf NASA93 (NASA data up to 1993):}


% 0 1 2 3 4 5 6 7 8 9=

{\scriptsize \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{darkgray}
\rowcolor[gray]{.9}  rank & treatment & median & IQR & \\%min= 14, max= 137\\
  1 &      COCOMO-II &    38  &  39 & \quart{4}{32}{19}{69} \\
  1 &   COCOMO-IIn/2 &    41  &  43 & \quart{8}{35}{21}{69} \\
  1 &   COCOMO-IIn/4 &    47  &  45 & \quart{9}{37}{26}{69} \\
%  1 &         cart &    49  &  57 & \quart{0}{46}{28}{69} \\
  1 & COCONUT:c*0.5,r=8n/2 &    54  &  50 & \quart{11}{41}{32}{69} \\
%  1 &     knear(1) &    56  &  77 & \quart{1}{63}{34}{69} \\
  1 & COCONUT:c*0.5,r=8 &    57  &  57 & \quart{8}{46}{34}{69} \\
  1 & COCONUT:c*0.5r=8n/4 &    58  &  45 & \quart{21}{37}{35}{69} \\
%  1 &       cart/2 &    65  &  112 & \quart{8}{91}{41}{69} \\
%  1 &       cart/4 &    68  &  74 & \quart{23}{60}{43}{69} \\
\end{tabular}}

% :learn 358.87023 :analyze 5.615541 :boots 1 effects 15 :conf 0.99

~\\

{\bf COC81 (original data from the 1981 COCOMO book):}


{\scriptsize \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
\arrayrulecolor{darkgray}
\rowcolor[gray]{.9}  rank & treatment & median & IQR & \\%min= 20, max= 281\\
  1 &      COCOMO-II &    33  &  35 & \quart{0}{13}{4}{30} \\
\hline  2 &   COCOMO-IIn/2 &    47  &  46 & \quart{2}{18}{10}{30} \\
  2 &   COCOMO-IIn/4 &    48  &  44 & \quart{3}{17}{10}{30} \\
  2 & COCONUT:c*0.5,r=8n/2 &    53  &  45 & \quart{5}{17}{12}{30} \\
  2 & COCONUT:c*0.5r=8n/4 &    57  &  44 & \quart{5}{17}{14}{30} \\
  2 & COCONUT:c*0.5,r=8 &    65  &  51 & \quart{4}{20}{17}{30} \\
%\hline  3 &         cart &    72  &  102 & \quart{9}{39}{19}{30} \\
%\hline  4 &       cart/4 &    75  &  214 & \quart{5}{82}{21}{30} \\
%  4 &       cart/2 &    80  &  151 & \quart{7}{58}{22}{30} \\
%  4 &     knear(1) &    87  &  236 & \quart{9}{90}{25}{30} \\
\end{tabular}}

 %:learn 173.557093 :analyze 9.017862 :boots 5 effects 14 :conf 0.9509900499
% noise


}
\caption{LOC noise results. MRE values. 
Displayed as per \fig{loc}.}\label{fig:noise}
\end{figure}


==> reviews-round0.tex <==
\newpage
\setcounter{page}{1}
\pagenumbering{roman}
\noindent
    {\bf REPLY TO REVIEWERS}

   \noindent
{\bf Comments from the special issue editor}

\begin{quote}{\em     The reviewers identify a number of strong points about your submission..}\end{quote}

\noindent
Thank you for that comment.

\begin{quote}{\em ... but also a number of issues related to presentation, emphasis (i.e., more emphasis of the 'negative' result is needed) and clarification of related work. Please take these comments into account when preparing your revision.}\end{quote}

\noindent We offer those those clarifications below, and several large changes:
\be
\item All the non-negative results in the last draft have been moved to another paper
  (so this paper now focuses on the negative);
\item Also removed were the experiments on errors in LOC (which is
  not really essential for our discussion).
  
\item
  At the suggestion of Reviewer\#2, we now include results from the
  \textit{Automatically Transformed Linear Baseline Model}(ATLM) proposed by Whigham et al. \cite{whigham15}.
\item Also, at the suggestion of Reviewer\#2, we pushed our business users to make
  more data available. We are happy to report that this draft now contains a full listing the Nasa10
  data set (that was unavailable to the general public at the time of writing the last draft).
\item Further, at the suggestion of Reviewer\#2, we re-ran all our results
  using another evalaution measure (not MRE). Those results did not change
  the conclusions of this paper... which is an interesting result in itself
  (different statistical measures are surprisingly blunt in the face
  of the large variances seen in effort estimation results). That finding (of
  equivalent conclusions despite different eval measures) is now on-line for
  you and the reviewers to inspect (at \url{http://tiny.cc/fb_rev2})-- but it adds no information to this
  paper (do not change any of our conclusions). We think we can write
  that up as a seperate paper so we ask that we do not
  present here.  Do you concur?
  \ee
  
\noindent
{\bf Comments to Reviewer\#1}

\noindent
Thank you for your details comments.  This new draft
contains many corrections and extensions as directed by your feedback.

All our changes are marked in the body of the paper in \textcolor{blue}{blue text}.
 

As to your specific comments: 
 
\begin{quote}{\em One of the puzzling claims of the paper is "For the non-COCOMO data sets, our newer estimation methods performed better than older methods". }. \end{quote}

\noindent
We have removed
that material.

\begin{quote}{\em ...more emphasis of the 'negative' result is needed}\end{quote}

\noindent
This was another good reason to remove the
non-COCOMO results).

\begin{quote}{\em There are more software engineering papers that have published errata in the recent years (but not necessarily via the main stream venues such as conferences and journals): JungWon Byun , SungYul Rhew, ManSoo Hwang, Vijayan Sugumaran, SooYong Park, SooJin Park Erratum to: Metrics for measuring the consistencies of requirements with objectives and constraints. Requirements Engineering March 2014, Volume 19, Issue 1`}\end{quote}

\noindent
That paper, at \url{http://tiny.cc/byun},
is an errata on the author names
and not on technical content. Hence, unless you direct us otherwise,
we will not reference that paper in this one.

\begin{quote}{\em Failure report, negative result and report on a previously published error are not the same; the introduction somehow puts them all together and tries to explain them with the same reasons.}\end{quote}



\noindent
That is an  important clarification.
We have fixed that, on \WHERE{Reviewer1a}.

\begin{quote}{\em "Secondly, it is not standard practice in software analytics for researchers to benchmark their latest results against some supposedly simpler "straw man" method." My guess would be that in many cases no such method is available making benchmarking impossible. When the domain starts to become more mature, this kind of comparisons are bing conducted (see, e.g., code cloning or a more recent work on tag inference for Stack Overflow posts).}\end{quote}

\noindent
Good comment--- which we've added
on \WHERE{Reviewer1b}.




\noindent
As to your specific comments, you write \begin{quote}{\em I'm
  also concerned about the choice of the
  datasets. Two of the datasets considered are
  affiliated with COCOMO, so they can provide a
  biased perspective on the power of the
  results. Are there additional datasets one might
  consider or are the COCOMO requirements so
  restrictive that no such datasets can be found
  unless at NASA?}. \end{quote}
 
 \noindent It is true that NASA contributed the data sets to NASA93 and NASA10.
  But for effects from non-NASA sources, we direct the reviewer to the 93 projects
  in the COC05
  results. Note that none of COC05 comes from NASA.

  Also, as I'm sure the reviewer knows,
  we have tried, most earnestly, for decades to collect
and publish  data sets (see the 
500+ data sets at \url{http://openscience.us}-- a web site we created and maintain for the SE community.
Even with that resources, and even after years of work,
these four data sets are all we can offer for this paper
(there are more, of course, but their users have declined
to let us use that other data).
 
  As to the ``NASA bias'' in the everything that is not COC05,
  in practice, very little software comes
``from NASA''. NASA is not
really a development organization. Rather it is a contractor
management site where the real work gets done by external
contractors (e.g. Rockwell Collins or Boeing). So a ``NASA app''
is really built by an exterior teams who delivers software
for many other applications and many other clients. Hence we argue
that lessons learned from data
marked as ``NASA'' actually applies
to a wide range of projects.
 
     \begin{quote}{\em The authors should have been more careful with introducing the techniques the use. It is not very clear what the "triangle function of Walkerden and Jeffery [68]" is precisely. Is it merely an idea that three variables should be combined as a weighted sum? Or is this a particular approach that can be used to derive coefficients 50, 33 and 17? I've checked the paper by Walkerden and Jeffery [68] but the triangle function is not mentioned.}\end{quote}

     \noindent You are right... we were far too clever in our write up at that
     point.
     P140 and p141 of the [68] describe how the estimates for the k-th
     nearest items are ranked according to the ordering of their items.
     What we should have written was $\frac{3a + 2b + 1c}{6}$. That has been fixed now on  \WHERE{Reviewer1c}.

     \begin{quote}{\em     Is $m.\mu$ the median of m (as suggested by the preceding discussion) or the mean of $m$ (as seems to follow from the paper by Mittas \& Angelis [52])?}\end{quote}

\noindent No... we wrote $\mu$ and we meant mean (as recommended by Mittas     \& Angelis).
 

\begin{quote}{\em 4.4 COCOMO with Incorrect Size Estimates ``That
  is, the parametric estimation method being
  recommended here is not unduly affected by noise
  where the KLOC values vary up to 50\% of their
  original value." I wonder whether one can expect
  estimation to be up to 50\% of the real
  value. Laranjeira in "Software Size Estimation of
  Object-Oriented Systems" (1990) has reported size
  estimates that were 3-4 times higher or lower than
  the actual system size; in two cases the estimates
  were as bas as 6 times off. This makes me wonder
  whether the "not unduly sensitive" in the
  conclusion does not overstate the results.}\end{quote}

\noindent Good catch- we increased the LOC estimation error study and found that
COCOMO breaks down when LOC errors grow beyond 200\% (but still worked up
to that point).

  Now we can include that result in this paper but, in keeping with the comments
about needing to focus the paper better, we have removed them.

 Please advise if you want the ``up to 200\%'' results returned to this paper.

\begin{quote}{\em Minor\newline
Section 3: reserach\newline
Section 4.3.4: thse\newline
Section 4.4: redundant )}\end{quote}

\noindent (and thanks for pointing out those errors).


\begin{quote}{\em The entire second half of the PDF contains the output of the LaTeX compilation. I presume that something went wrong during the submission process.}\end{quote}

\noindent Yes, that was strange. Sorry you had to deal with that.

\noindent
{\bf Comments to Reviewer\#2}

\noindent
Thank you for your details comments.  This new draft
is significantly improved thanks to your  feedback. 

All our changes are marked in the body of the paper in \textcolor{blue}{blue text}.
Several large (and confusing) parts of the previous draft have been deleted since,
as you wrote:

\begin{quote}{\em  Generally, the paper has a large number of different elements  that makes it difficult to follow. If you are interested in the value of COCOMO-II why not stick to that.
}\end{quote}

At your suggestion, to clarify and focus the paper we have removed (a)~all the non-COCOMO results;
and (b)~all the COCOMO size error results.

Also, at your suggestion, we ran more experiments (with different error measures,
with the Whigham methods, using Effort/FP). As remarked below, those
changes did not change our conclusions. Nevertheless, it was useful proposing
those new experiments since it increases the external validity of this paper.

As to your specific comments:

\begin{quote}{\em A ``strawman" should not be something that is so
  foolish that it is impossible not to
  outdo. Researchers in the past have used simple
  regression without a logarithmic transformation
  and MMRE as an accuracy measure for comparison
  with new estimation methods.  Kitchenham \& Mendes
  pointed out this was not a valid approach.}\end{quote}

Thank you for the reference to the ATLM method from
the Whigham paper (Whigham, P., Owen, C., and
Macdonell, S. A baseline model for software effort
estimation. ACM Trans. on Softw. Eng. \&
Methodol. 24, 3 2015). We agree that the literature
agrees that ATLM is a suitable ``straw man''. We
have included those results in this paper in
\WHERE{Reviewer2c}, \WHERE{Reviewer2e} and \WHERE{Reviewer2f}.

Just on the side node, thanks for pointing us to
the  Whigham paper. It turns out that  as a baseline method,
it performs much worse than anything else we tried. So now we have another paper
to write after this one ``A Better Baseline for Effort Estimation''-- which would
not be happening without your input.

For now, what we can say in this paper (which is a clear negative report) is
that nothing we've tried (including the Whigham baseline and
all the supposedly clever implementations
we've built in the last decade) perform any better than old fashioned COCOMO.

\begin{quote}{\em RQ1 I don't think the issue was ever about "just lines of code" it was about simple regression rather than a complex  deterministic model. }\end{quote}

Actually, our experience is a little different from yours on this point.
I've been at SE conferences where Martin Shepperd  has said exactly that COCOMO
runs no better than simple LOC.

\begin{quote}{\em However,  the function point community do recommend the taking the average of the productivity (Effort/FP) then multiplying by the FP estimate of a project needing a cost estimate.}\end{quote}

Thank you for that suggestion. We tried that treatment of  effort
and found it made all our predictions much worse. For those results,
please  see \url{http://tiny.cc/e_prod}.  


\begin{quote}{\em 
  This paper uses two proprietary data sets which means the results cannot be independently validated. This is not very satisfactory. We have too many data mining studies that cannot be reproduced....
The results for NASA 10 and COC05 are hearsay.}\end{quote}

We took your comment back to our business users and can report some success there (thank you for your comment).
NASA10 is now publicly available (and included in this paper, \WHERE{Reviewer2b}).

As to the remaining data set (COC05),
we agree that it is not ideal that it remains closed source.  But
we also think that it is not fatal to this paper. 
Other empirical software engineering researchers publish
results with a clear organizational bias (witness the results
of Zimmermann and Bird from Microsoft data
or Penix and Elbaum working from Google data). What is important, and what is done by Zimmermann, Bird,
Penix, Elbaum and this paper is to clearly state the source of any such bias.

\begin{quote}{\em Figure 2 . The Coc81 data set has 63 projects (or did you remove one of them?)}\end{quote}

\noindent Our mistake. fixed.

\begin{quote}{\em Jorgensen didn't talk about "Delphi-based" methods he talked about  "expert-based" estimation.}\end{quote}

\noindent You are right.. ``expert'' is a better term than Delphi. We have changed all those terms here.


\begin{quote}{\em Equation (3) You should not be using the biased
  MRE measure. The poor behavior of MRE has been
  well documented in leading journals (see ref [1],
  [3] \& [4]. It doesn't matter whether you use the
  median or mean MRE the metric is still
  biased.

  If you really want a measure between 0 and 1 to
  assess performance, use an R-squared equivalent
  such as the ratio of the squared difference
  between the estimate and actual divided by the
  squared difference between the actual and the
  average effort.  }\end{quote}

\noindent As part of a revised threats to validity section on \WHERE{Reviewer2d}, we 
re-run all the experiments using the measure you propose $r2=\abs{\frac{a^2-e^2}{a^2 - \overline{a}^2}}$.
A sample of those results are shown in this paper 
In summary, the change of evaluation measure
changed our conclusions not at all, something we commented on 
at \WHERE{Reviewer2g}. 

In the text of this paper we   include one chart comparing $e2$ to MRE
(and the rest of those comparisons are available for
your  inspection at \url{http://tiny.cc/fb_rev2}). 


If you prefer,  we could add all the $r2$ to this paper.
But since there is no conclusion change between MRE and $r2$, and since there is consensus amongst this paper's
reviewers that the old draft had too much in it, we think we should not
add  more experimental detail that
only makes the same conclusions.


\begin{quote}{\em Whigham et al.'s default model seems more
  appropriate as a useful strawman and is certainly
  better than lines of code.}\end{quote}

 We agree and 
have included those results from the Whigham this paper at
\WHERE{Reviewer2c}, \WHERE{Reviewer2e} and \WHERE{Reviewer2f}. And please note, as we stated
before, how badly
Whigham performs in \WHERE{Reviewer2e}-- thanks to your comments on this matter, we now have
another paper to write about a better baseline for effort estimation.


\begin{quote}{\em From your description it appears that TEAK
  removes projects - how then do you do a fair
  comparison with other methods ? }\end{quote}

\noindent Note that TEAK and PEEKING2 only prunes the training set, not the test set so it is a fair comparison.
We have added a note to this effect at \WHERE{Reviewer2d}.

\begin{quote}{\em Since Barry Boehm is a co-author, it should be simple to confirm whether or not any of the NASA93 projects were used in the construction of COCOMO-II.}\end{quote}

\noindent We double checked the raw data (KLOCs and effort)
and can confirm that none of NASA93 was uses
to tune COCOMO 2000 (a comment we add at 
\WHERE{Reviewer2a}).


\begin{quote}{\em  4.3.1 This seems like a good idea. There are too many levels (which should be treated as dummy variables) for a data-based calibration process to work well without a very large data base.}\end{quote}

\noindent
Thank you for that comment. We agree.

\begin{quote}{\em 4.4 It would be useful to plot the actual size against the recalculated size. If the revised size is still correlated with the actual size you may only have demonstrated that the exponential term in the COCOMO model is close to 1.}\end{quote}

\noindent
This remark refers to material that has now been deleted from this version.
Please see above discussion with Reviewer1 on `` 4.4 COCOMO with Incorrect Size Estimates ''.
In order to focus the paper better,  have removed it from this draft. However, at your direction, we would gladly return it.


\begin{quote}{\em Section 5: I am not clear why the authors felt it necessary to include Figures 13 \& 14 other than to have something positive to report. However, there does not appear to be much difference between PEEKING2 and Knear(3) at least not really sufficient to claim that PEEKING2 performed best.}\end{quote}

\noindent We concur. We have removed that entire section about positive results on non-COCOMO data.
The resulting paper is much clear, in our opinion.

As a final note, thank you again for your comments. This draft is now 6 pages shorter (since it has dispensed
with much superfluous material), contains numerous important extensions (e.g. the full inclusion of the Nasa10 data),
as well as important comments on external validity and other matters.
\newpage

==> reviews-round1.tex <==
\newpage
\setcounter{page}{1}
\pagenumbering{roman}
\noindent
    {\bf REPLY TO REVIEWERS}

\subsection*{Comments from editor}

\noindent
{\em Thanks for your re-submission. Please review the following minor comments when re-submitting your manuscript.}

We trust that this
new draft addresses the remaining reviewer concerns.
\subsection*{Reviewer \#1}

\noindent{\em The authors have adequately addressed most of my comments. Publication of the NASA10 dataset is a valuable addition to the effort estimation data.}

Thank you for that comment


\noindent{\em p.8 Fig.5 What is xhigh? Why are some parameters scored on the five-point scale and some others on a six-point scale (the paper mentions the five-point scale only).}

Caption of Fig.5 extended with those definitions.

\noindent{\em p.10 effort in (5) should be typeset differently}

You are quite correct. Now fixed.

\noindent{\em p.11-12 Discussion of the Scott-Knott procedure should be more elaborate. How are the rx treatments in the example related to l, m and n from the preceding explanation?  }


We've rewritten the text at the start of section 3.3 to better illustrate that nomenclature using some
example from our RQ1 results.


\subsection*{Reviewer \#2}
\noindent{\em There do seem to be a few outstanding issues;}

\noindent{\em 1. Page 2 Lines 27-30 It surprising that the authors have decided to use Whingham et al.'s benchmark, but do not note that their study was motivated by a failure to replicate previous studies.}

Added.


\noindent{\em 2. The authors seem to have got the equation for R2 (the Multiple Correlation Coefficient) wrong. Its 1 - the SUM of the squared differences between the each actual and its predicted value divided by the SUM of the squared differences between the actuals and the average of the actuals. (By squaring the differences you avoid the need for applying the abs function.) It is interpreted as proportion of the variance in the outcome variable accounted for by the model. I am sorry I didn't specify it exactly but its hard to specify equations in text. See http://imgur.com/a/f3oAm }

Fixed. Sorry for that error.

\noindent{\em 3. MRE should be depreciated in all cost estimation studies because it can be biased. Its major problems occur when researchers use machine learning methods and adopt MRE as a fitness function which will lead to developing predictions that are biased towards underestimation but will have "better" values of MRE than unbiased models. Its not a problem if you use statistically derived models because they are always unbiased (I understood that COCOMO-II used a Bayesian development method, so it should produce unbiased estimates). Nonetheless we should NOT encourage other researchers to use a metric that can be unreliable. }

As per your suggestion, we have switched to SE \eq{se}.

\subsection*{Reviewer \#3}

Thank you you for the clarity of your forthright comments. We
respond below in the same honest and forthright manner.

\noindent{\em The premise that COCOMO inputs are available remains an unnecessary burden to limit this research. This assumption immediately biases the research comparison and limits the comparison to what many practitioners would expect, knowing that there a many different estimation methods and tools in widespread use today.}

Respectfully, we must disagree. COCOMO is {\bf not} an unnecessary burden. We show in {\bf RQ4} that we can run COCOMO with up to half the COCOMO
input missing and using just a few examples.

Also, in our experience, with one exception it takes about an hour to a half day to collect COCOMO data per project (given access to local developers).
The one exception is accessing the actual development effort-- which is a problem not just for COCOMO
but for many estimation modeling methods.

\noindent{\em 2) A proper comparison that I had expected to see was a comparison of the most widely adopted tools and methods in use today using real data sets collected in the recent past.  The research could then be more generalizable and not suffer the extent of internal and external validity suffered by this research as is.}

Please recall that an earlier version of this
paper had something like that-- we had a final
section offering recommendations of what was ``best of breed'' for non-COCOMO data sets. But reviewers
in prior rounds asked us to remove that section in order to better focus the paper.


\noindent{\em 3) Most of the second paragraph of the Introduction section (beginning with numbered line 12)is unnecessarily provocative and advertises the author's bias,}

Well, certainly, any text can be improved with editing and we could
cut the material shown below in blue. However, we disagree with this
reviewer on the value of this text. This revision includes all the following
text and we recommend that the paper be accepted with that text.

 
\begin{quote}{\textcolor{blue}{
\bi
\item
``This conclusion comes with two caveats. Firstly, not all projects can be expressed in terms of COCOMO– but when there is a choice, the results of this paper argue that there is value in using that format. Secondly, our conclusion is about solo prediction methods which is different to the ensemble approach [35, 48, 53, 54]– but if using ensembles, this paper shows that parametric estimation would be a viable ensemble member.''
\item
``For pragmatic and methodological reasons,it is important to report negative results like the one described above. Pragmatically, it is important for industrial practitioners to know that (sometimes) they do not need to waste time straining to understand bleeding-edge technical papers. In the following, we precisely define the class of project data that does not respond well to bleeding-edge effort estimation techniques. For those kinds of data sets,practitioners can be rest assured that it is reasonable and responsible and useful to use simple traditional methods.''
\item ``Also,'' 
\ei}}
\end{quote}

\noindent{\em 4) The third paragraph beginning at numbered line 19 seems out of place and unconnected with the discussion.   It would help if there was a leading or summary sentence that cemented the place this paragraph should take in the overall story of the paper.}

We do not agree that it is out of place.

\noindent{\em 5) On numbered line 48 of the Introduction section, a very strong "if" occurs which seems unreasonable.}

Given the results of this paper, we might expect more ways to satisfy this ``if''.


\noindent{\em 6) On page 3, the four research questions should be restated to replace parametric estimation with "COCOMO".  It is quite bold to presume that COCOMO represents the entire class of parametric models for SEE considering the widespread adoption of PRICE-S, SEER-SEM, and SLIM.}

Beg pardon, and sorry to keep disagreeing with you,
but     there is a known very 
strong association between these models.
Ray Madachy's paper http://csse.usc.edu/TECHRPTS/2008/usc-csse-2008-816/usc-csse-2008-816.pdf
compares COCOMO-II with SEER-SEM and Price-S (now called True S), which mentioned that the underlying cost estimation relationships in SEER-SEM and true S share  common aspects with COCOMO-II, though each offer some difference commercial features. See section 2.1 for further info.

So our opinion is that it is valid
to assert that COCOMO is an example of parametric estimation.


\noindent{\em I would have preferred to see these other models included in the research because they represent the ongoing research and embodiment in the form of the latest in commercial tools for SEE.}

Please see our reply to point 2.

\noindent{\em 7) Page 6 also seems to ignore these other SEE models and tools which are quite popular.}


Please see our reply to point 2.

\noindent{\em 8) On page 10 in section 3.1, the "Ecological inference" statement seems to be in conflict with Simpson's Paradox.}

Yes, it is true that effort estimation data
has certain properties not found in distributions
from other domains. For more on this, please see
where we show that bias and variance is NOT altered
in effort estimation if we move from leave-one-out to cross-val. http://www.sciencedirect.com/science/article/pii/S0164121213000538

\noindent{\em 9) On page 17 in section 5.0, the threats to validity should outline the threats previously listed in this comment section.}

If you are referring here to our use of COCOMO as the baseline starting
point for this study, then referring back to our earlier replies
(above), COCOMO is not a crippling limiting assumption to the external
validity of this work.

\noindent{\em 10) I would like to commend the use of the Scott-Knott clustering algorithm as an improvement over other methods suffering from overlapping, to include the popular Tukey method.}

Thank you for that comment


